PerfSeer: An Efficient and Accurate Deep Learning Models Performance Predictor

Predicting the performance of deep learning (DL) models, such as execution time and resource utilization, is crucial for Neural Architecture Search (NAS), DL cluster schedulers, and other technologies that advance deep learning. The representation of a model is the foundation for its performance prediction. However, existing methods cannot comprehensively represent diverse model configurations, resulting in unsatisfactory accuracy. To address this, we represent a model as a graph that includes the topology, along with the node, edge, and global features, all of which are crucial for effectively capturing the performance of the model. Based on this representation, we propose PerfSeer, a novel predictor that uses a Graph Neural Network (GNN)-based performance prediction model, SeerNet. SeerNet fully leverages the topology and various features, while incorporating optimizations such as Synergistic Max-Mean aggregation (SynMM) and Global-Node Perspective Boost (GNPB) to capture the critical performance information more effectively, enabling it to predict the performance of models accurately. Furthermore, SeerNet can be extended to SeerNet-Multi by using Project Conflicting Gradients (PCGrad), enabling efficient simultaneous prediction of multiple performance metrics without significantly affecting accuracy. We constructed a dataset containing performance metrics for 53k+ model configurations, including execution time, memory usage, and Streaming Multiprocessor (SM) utilization during both training and inference. The evaluation results show that PerfSeer outperforms nn-Meter, Brp-NAS, and DIPPM.

==> equation/metrics.tex <==
\begin{align}
  % \begin{split}
    \text{MAPE} &= \frac{1}{n}\sum_{i=1}^{n}\frac{error_i}{y_i}\times 100\% \\
    x\%\text{Acc} &= \frac{1}{n}\sum_{i=1}^{n}(\begin{cases} 
    1 & \text{if } \frac{{error}_i}{y_i} \leq x\% \\
    0 & \text{otherwise}
    \end{cases}) \times 100\% \\
  % \end{split}
  % \begin{split}
    \text{RMSPE} &= \sqrt{\frac{1}{n}\sum_{i=1}^{n}\left(\frac{error_i}{y_i}\right)^2} \times 100\% \\
  % \end{split}
  \label{eq:metrics}
  \nonumber
\end{align}

==> equation/nnm.tex <==
\begin{equation}
\text{SynMM}(\bar{\vv}_1, \bar{\vv}_2) = \text{Linear}\left(\bar{\vv}_1 \cat \bar{\vv}_2\right),
\end{equation}
% \vspace{-10pt}  
\begin{equation}
    \bar{\vv}_1 = \text{Max}(V) = \max _{\vv_i \in V} \vv_i,
\end{equation}
% \vspace{-10pt}  
\begin{equation}
     \bar{\vv}_2 = \text{Mean}(V) = \frac{1}{N^v} \sum_{\vv_i \in V} \vv_i.
\end{equation}
 

==> figure/4-general_model.tex <==
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figure/src/4-general_model.pdf}
    \caption{General architecture of CNNs in the dataset.}
    \label{fig:general model}
\end{figure}

==> figure/5-evaluation_overview.tex <==
\begin{figure}[htb]
  \centering
  \includegraphics[width=1.0\columnwidth]{figure/src/5-evaluation_overview.pdf}
  \caption{Predicted performance metrics versus measured performance metrics. 
    The points falling on the x\% error area represent that the absolute error of the prediction of the sample is within the absolute error bound x\%.
    % Additionally, due to the large size of the test set, only 2000 randomly sampled samples are displayed in the figure, with the value in brackets calculated from the complete test set.
    }
  \label{fig:evaluation overview}
\end{figure}

==> table/collectbed.tex <==
\begin{table}[htb]
\caption{Hardware and software setup of performance metrics collection.}
\label{tab:collectbed}
\belowrulesep=0pt
\aboverulesep=0pt
    \renewcommand{\arraystretch}{1}
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{lll}
    
    \specialrule{1.5pt}{0pt}{0pt}
    Type & Name & Description \\
    \specialrule{1.0pt}{0pt}{0pt}
    
    \multirow{2}{*}{Hardware} 
    % & Type & Type(e.g., Conv2D and Linear) \\
    & CPU & Intel(R) Xeon(R) Gold 6226R \\
    & GPU & NVIDIA GeForce RTX 3090 \\
    \specialrule{1.0pt}{0pt}{0pt}
    
    \multirow{3}{*}{Software} 
    & Operating system & Ubuntu 20.04 \\
    & CUDA & CUDA 11.7 \& cuDNN 8.5.0 \\
    & DL framework & PyTorch-1.13.0+cu117 \\
    \specialrule{1.5pt}{0pt}{0pt}
    
    \end{tabular}}
\end{table}

==> table/datasets.tex <==
\begin{table*}[htb]
\caption{Dataset profile. 
In this paper, Util, Mem, and Time refer to the GPU SM utilization, GPU memory usage, and execution time of each iteration for training or inference of DL models, respectively. 
% Additionally, the data in this table is based on the model's statistics for different batch sizes, not limited to the default batch size of 1. Therefore, this may result in relatively larger values for metrics such as FLOPs.
Additionally, the data comes from models with different batch sizes, not just the default of 1, which may lead to larger statistical values (e.g., FLOPs).
}
\label{tab:datesets profile}
\belowrulesep=0pt
\aboverulesep=0pt
    \renewcommand{\arraystretch}{1.0}
    \resizebox{2.0\columnwidth}{!}{
    \begin{tabular}{cccccccccc}
    
    \specialrule{1.5pt}{0pt}{0pt}
    % summury title
    \multirow{2}{*}{Statistics} & \multirow{2}{*}{FLOPs$[ \text{G} ]$} & \multirow{2}{*}{MAC$[ \text{GBytes} ]$} & \multirow{2}{*}{Params$[ \text{M} ]$} & \multicolumn{3}{c}{Training} & \multicolumn{3}{c}{Inference} \\
    % half mid line
    \cmidrule(lr){5-7} \cmidrule(lr){8-10}
    
    %% title
    & & & & {Util$[ \text{\%} ]$} & {Mem$[ \text{MBytes} ]$} & {Time$[ \text{ms} ]$} & {Util$[ \text{\%} ]$} & {Mem$[ \text{MBytes} ]$} & {Time$[ \text{ms} ]$} \\
    \specialrule{1.0pt}{0pt}{0pt}
    
    Mean & 214.8 & 7.7 & 9.5 & 62.4 & 5,255 & 87.1 & 72.9 & 2,412 & 23.8 \\
    Min & 0.05 & 0.01 & 0.04 & 5.0 & 1,500 & 2.9 & 8.0 & 1,410 & 0.8 \\
    Median & 40.8 & 2.1 & 3.6 & 66.9 & 2,728 & 44.1 & 97.0 & 1,790 & 9.2 \\
    Max & 22,543.9 & 70.2 & 254.9 & 99.0 & 24,244 & 1,919.5 & 99.0 & 19,462 & 554.5 \\
    \specialrule{1.5pt}{0pt}{0pt}
    
    \end{tabular}}
\end{table*}

